Relightable Full-Body Gaussian Codec Avatars

We propose Relightable Full-Body Gaussian Codec Avatars, a new approach for modeling relightable full-body avatars with fine-grained details including face and hands. The unique challenge for relighting full-body avatars lies in the large deformations caused by body articulation and the resulting impact on appearance caused by light transport. Changes in body pose can dramatically change the orientation of body surfaces with respect to lights, resulting in both local appearance changes due to changes in local light transport functions, as well as non-local changes due to occlusion between body parts. To address this, we decompose the light transport into local and non-local effects. Local appearance changes are modeled using learnable zonal harmonics for diffuse radiance transfer. Unlike spherical harmonics, zonal harmonics are highly efficient to rotate under articulation. This allows us to learn diffuse radiance transfer in a local coordinate frame, which disentangles the local radiance transfer from the articulation of the body. To account for non-local appearance changes, we introduce a shadow network that predicts shadows given precomputed incoming irradiance on a base mesh. This facilitates the learning of non-local shadowing between the body parts. Finally, we use a deferred shading approach to model specular radiance transfer and better capture reflections and highlights such as eye glints. We demonstrate that our approach successfully models both the local and non-local light transport required for relightable full-body avatars, with a superior generalization ability under novel illumination conditions and unseen poses.

==> a3_limitations.tex <==
Our method has several limitations.  First, the
cloth dynamics are based purely on the learned latent space, which may not be
physically plausible.  In such a case, the method may fail in
out-of-distribution scenarios, \eg\ when hands are touching the cloth or when
extreme body poses are present.  A more physically plausible clothing layer~\cite{Xiang2023DrivableAC,Xiang2022DressingA,Rong2024ARXIV,Peng2024ARXIV,Zheng2024ECCV}
could be potentially integrated to resolve this issue.
Second, our method is still suboptimal in
capturing detailed appearances of eyes, faces, and hands compared to specialized
methods~\cite{li2022eyenerf,Saito2024CVPR,Chen2024CVPR,Iwase2023CVPR}, as the
model capacity assigned to these regions is limited.  This could be potentially solved
by dynamically assigning UV space capacity to different body parts during learning.
Lastly, our method has
limited scalability as it requires a multi-camera setup with known light sources, a natural future direction is to extend the method to universal setups
similar to related face~\cite{Li2024SIGGRAPHASIA} and hand~\cite{Chen2024CVPR} models.
